Leveraging Community and Author Context to Explain the Performance and Bias of Text-Based Deception Detection Models

Deceptive news posts shared in online communities can be detected with NLP models, and much recent research has focused on the development of such models. In this work, we use characteristics of online communities and authors -- the context of how and where content is posted -- to explain the performance of a neural network deception detection model and identify sub-populations who are disproportionately affected by model accuracy or failure. We examine who is posting the content, and where the content is posted to. We find that while author characteristics are better predictors of deceptive content than community characteristics, both characteristics are strongly correlated with model performance. Traditional performance metrics such as F1 score may fail to capture poor model performance on isolated sub-populations such as specific authors, and as such, more nuanced evaluation of deception detection models is critical.

==> figs/token_correlations_table.tex <==
\tiny
\begin{tabular}{@{\hskip -.05cm}l@{\hskip .0cm}r@{\hskip .05cm}|rr|rr|rr}
\toprule 
 & & \multicolumn{2}{c|}{Uses of} & \multicolumn{2}{c|}{Frequency} & \multicolumn{2}{c}{Correlation ($r$)}\\
 && \multicolumn{2}{c|}{N-Gram} & \multicolumn{2}{c|}{(\% of posts)} & \multicolumn{2}{c}{w/ Correctness}\\
{} &&   {\bf Total} &   {\bf \% D} & 
{\bf D Posts}&{\bf T Posts}& 
 {\bf $r_D$} &    {\bf $r_T$} \\
% & & \multicolumn{2}{c|}{Use of N-Gram} & \multicolumn{2}{c|}{Frequency in Posts}& \multicolumn{2}{c}{Correlation with Correct}\\
%                         &         &   {Total} &   {\% Deceptive} &   {\% of D Posts} &   {\% of T Posts} &                            {$r$ w/ Deceptive} &                              {$r$ w/ Trusted} \\
\midrule
%\multirow{2}{*}{ {>90\% Deceptive}} 
&  {podesta} &          44 &     97.7 &                 1.8 &               0.0 &  \cellcolor[rgb]{0.949,0.966,0.924} +0.06 &  \cellcolor[rgb]{0.971,0.960,0.966} -0.02 \\
              &  {breitbart} &          53 &     92.5 &                 2.0 &               0.1 &  \cellcolor[rgb]{0.946,0.966,0.918} +0.06 &  \cellcolor[rgb]{0.974,0.949,0.962} -0.05 \\
%\cline{1-8}
%\multirow{19}{*}{ {70-90\% Deceptive}} 
&  {wikileaks} &          95 &     88.4 &                 3.4 &               0.4 &  \cellcolor[rgb]{0.941,0.965,0.906} +0.09 &  \cellcolor[rgb]{0.977,0.935,0.957} -0.08 \\
              &  {clinton campaign} &          30 &     86.7 &                 1.1 &               0.1 &  \cellcolor[rgb]{0.957,0.967,0.942} +0.04 &  \cellcolor[rgb]{0.969,0.967,0.968} -0.01 \\
              &  {dnc} &          55 &     85.5 &                 1.9 &               0.3 &  \cellcolor[rgb]{0.952,0.967,0.930} +0.05 &  \cellcolor[rgb]{0.973,0.953,0.963} -0.04 \\
              &  {hillarys} &          38 &     84.2 &                 1.3 &               0.2 &  \cellcolor[rgb]{0.952,0.967,0.930} +0.05 &  \cellcolor[rgb]{0.976,0.942,0.959} -0.06 \\
\ignore{              &  {emails} &          72 &     79.2 &                 2.3 &               0.6 &  \cellcolor[rgb]{0.946,0.966,0.918} +0.07 &  \cellcolor[rgb]{0.977,0.935,0.957} -0.08 \\
              &  {email} &          76 &     78.9 &                 2.4 &               0.6 &  \cellcolor[rgb]{0.949,0.966,0.924} +0.06 &  \cellcolor[rgb]{0.976,0.942,0.959} -0.06 \\
              &  {hillary} &         418 &     77.3 &                13.2 &               3.5 &  \cellcolor[rgb]{0.931,0.964,0.882} +0.11 &  \cellcolor[rgb]{0.988,0.896,0.943} -0.16 \\
              &  {speech} &          34 &     76.5 &                 1.1 &               0.3 &  \cellcolor[rgb]{0.962,0.968,0.954} +0.02 &  \cellcolor[rgb]{0.967,0.968,0.966} +0.01 \\
              &  {for hillary} &          33 &     75.8 &                 1.0 &               0.3 &  \cellcolor[rgb]{0.957,0.967,0.942} +0.04 &  \cellcolor[rgb]{0.976,0.939,0.958} -0.06 \\
              &  {syria} &          38 &     73.7 &                 1.1 &               0.4 &  \cellcolor[rgb]{0.952,0.967,0.930} +0.05 &  \cellcolor[rgb]{0.977,0.935,0.957} -0.07 \\
              &  {foundation} &          34 &     73.5 &                 1.0 &               0.3 &  \cellcolor[rgb]{0.954,0.967,0.936} +0.04 &  \cellcolor[rgb]{0.976,0.942,0.959} -0.05 \\
              &  {john} &          45 &     73.3 &                 1.3 &               0.4 &  \cellcolor[rgb]{0.954,0.967,0.936} +0.04 &  \cellcolor[rgb]{0.957,0.967,0.942} +0.03 \\
              &  {muslim} &          65 &     72.3 &                 1.9 &               0.7 &  \cellcolor[rgb]{0.957,0.967,0.942} +0.04 &  \cellcolor[rgb]{0.973,0.953,0.963} -0.03 \\
              &  {hillary clinton} &         204 &     72.1 &                 6.0 &               2.1 &  \cellcolor[rgb]{0.946,0.966,0.918} +0.07 &  \cellcolor[rgb]{0.983,0.914,0.950} -0.12 \\
              &  {matter} &          35 &     71.4 &                 1.0 &               0.4 &  \cellcolor[rgb]{0.957,0.967,0.942} +0.03 &  \cellcolor[rgb]{0.970,0.963,0.967} -0.01 \\
              &  {breaking} &          38 &     71.1 &                 1.1 &               0.4 &  \cellcolor[rgb]{0.967,0.968,0.966} +0.01 &  \cellcolor[rgb]{0.972,0.956,0.964} -0.03 \\
              &  {want} &          51 &     70.6 &                 1.5 &               0.6 &  \cellcolor[rgb]{0.967,0.968,0.966} +0.00 &  \cellcolor[rgb]{0.959,0.968,0.948} +0.02 \\
              &  {party} &          51 &     70.6 &                 1.5 &               0.6 &  \cellcolor[rgb]{0.965,0.968,0.960} +0.01 &  \cellcolor[rgb]{0.969,0.967,0.968} -0.01 \\
              &  {cruz} &          44 &     70.5 &                 1.3 &               0.5 &  \cellcolor[rgb]{0.957,0.967,0.942} +0.03 &  \cellcolor[rgb]{0.977,0.935,0.957} -0.07 \\
}
\cline{1-8}
\ignore{
%\multirow{12}{*}{ {70-90\% Trusted}} 
&  {made} &          41 &     29.3 &                 0.5 &               1.1 &  \cellcolor[rgb]{0.970,0.963,0.967} -0.01 &  \cellcolor[rgb]{0.959,0.968,0.948} +0.02 \\
              &  {said} &          46 &     28.3 &                 0.5 &               1.2 &  \cellcolor[rgb]{0.962,0.968,0.954} +0.02 &  \cellcolor[rgb]{0.954,0.967,0.936} +0.04 \\
              &  {tax} &          40 &     27.5 &                 0.4 &               1.1 &  \cellcolor[rgb]{0.969,0.967,0.968} -0.00 &  \cellcolor[rgb]{0.954,0.967,0.936} +0.05 \\
              &  {pay} &          43 &     25.6 &                 0.4 &               1.2 &  \cellcolor[rgb]{0.971,0.960,0.966} -0.02 &  \cellcolor[rgb]{0.946,0.966,0.918} +0.07 \\
              &  {brexit} &          41 &     24.4 &                 0.4 &               1.2 &  \cellcolor[rgb]{0.976,0.942,0.959} -0.06 &  \cellcolor[rgb]{0.949,0.966,0.924} +0.06 \\
              &  {north} &          46 &     21.7 &                 0.4 &               1.3 &  \cellcolor[rgb]{0.969,0.967,0.968} -0.01 &  \cellcolor[rgb]{0.957,0.967,0.942} +0.03 \\
              &  {china} &          47 &     21.3 &                 0.4 &               1.4 &  \cellcolor[rgb]{0.971,0.960,0.966} -0.02 &  \cellcolor[rgb]{0.970,0.963,0.967} -0.01 \\
              &  {uk} &          54 &     20.4 &                 0.4 &               1.6 &  \cellcolor[rgb]{0.959,0.968,0.948} +0.03 &  \cellcolor[rgb]{0.971,0.960,0.966} -0.02 \\
              &  {city} &          40 &     20.0 &                 0.3 &               1.2 &  \cellcolor[rgb]{0.967,0.968,0.966} +0.01 &  \cellcolor[rgb]{0.954,0.967,0.936} +0.05 \\
}
              &  {til} &         125 &     17.6 &                 0.9 &               3.8 &  \cellcolor[rgb]{0.988,0.893,0.942} -0.16 &  \cellcolor[rgb]{0.915,0.962,0.846} +0.16 \\
              &  {bbc} &          43 &     14.0 &                 0.2 &               1.4 &  \cellcolor[rgb]{0.979,0.928,0.954} -0.09 &  \cellcolor[rgb]{0.944,0.966,0.912} +0.08 \\
              &  {til that} &          37 &     13.5 &                 0.2 &               1.2 &  \cellcolor[rgb]{0.980,0.924,0.953} -0.10 &  \cellcolor[rgb]{0.941,0.965,0.906} +0.08 \\
%\cline{1-8}
%\multirow{2}{*}{ {>90\% Trusted}} 
&  {climate} &          29 &      6.9 &                 0.1 &               1.0 &  \cellcolor[rgb]{0.965,0.968,0.960} +0.01 &  \cellcolor[rgb]{0.946,0.966,0.918} +0.07 \\
              &  {bbc news} &          29 &      0.0 &                 0.0 &               1.1 &    \cellcolor[rgb]{0.890,0.890,0.890} N/A &  \cellcolor[rgb]{0.946,0.966,0.918} +0.07 \\
\bottomrule
\end{tabular}

==> figs/top_ngrams_table.tex <==
\tiny
    %\centering
    \begin{tabular}{r|@{\hskip .05cm}rr|rr|rr}
\toprule
 & \multicolumn{2}{c|}{Uses of} & \multicolumn{2}{c|}{Frequency} & \multicolumn{2}{c}{Correlation ($r$)}\\
 & \multicolumn{2}{c|}{N-Gram} & \multicolumn{2}{c|}{(\% of posts)} & \multicolumn{2}{c}{w/ Correctness}\\
{} &  \textbf{Total} &  \textbf{\% D} & 
{\bf D Posts}&{\bf T Posts}&
%{\begin{tabular}{r} \textbf{\% D}\\{\bf Posts} \end{tabular}} & 
%\begin{tabular}{r} \textbf{\% T}\\{\bf Posts} \end{tabular} & 
\textbf{$r_D$} &   \textbf{$r_T$} \\
\midrule
trump           &         785 &     49.7 &                15.9 &              14.7 &  \cellcolor[rgb]{0.979,0.928,0.954} -0.09 &  \cellcolor[rgb]{0.970,0.963,0.967} -0.01 \\
clinton         &         492 &     66.3 &                13.3 &               6.2 &  \cellcolor[rgb]{0.954,0.967,0.936} +0.04 &  \cellcolor[rgb]{0.983,0.914,0.950} -0.12 \\
hillary         &         418 &     77.3 &                13.2 &               3.5 &  \cellcolor[rgb]{0.931,0.964,0.882} +0.11 &  \cellcolor[rgb]{0.988,0.896,0.943} -0.16 \\
us              &         305 &     51.5 &                 6.4 &               5.5 &  \cellcolor[rgb]{0.954,0.967,0.936} +0.05 &  \cellcolor[rgb]{0.977,0.935,0.957} -0.08 \\
says            &         252 &     31.7 &                 3.3 &               6.4 &  \cellcolor[rgb]{0.970,0.963,0.967} -0.01 &  \cellcolor[rgb]{0.952,0.967,0.930} +0.05 \\
donald          &         234 &     39.3 &                 3.8 &               5.3 &  \cellcolor[rgb]{0.979,0.928,0.954} -0.09 &  \cellcolor[rgb]{0.954,0.967,0.936} +0.04 \\
new             &         225 &     44.0 &                 4.0 &               4.7 &  \cellcolor[rgb]{0.972,0.956,0.964} -0.03 &  \cellcolor[rgb]{0.969,0.967,0.968} -0.01 \\
hillary clinton &         204 &     72.1 &                 6.0 &               2.1 &  \cellcolor[rgb]{0.946,0.966,0.918} +0.07 &  \cellcolor[rgb]{0.983,0.914,0.950} -0.12 \\
sanders         &         203 &     56.7 &                 4.7 &               3.3 &  \cellcolor[rgb]{0.976,0.942,0.959} -0.06 &  \cellcolor[rgb]{0.971,0.960,0.966} -0.02 \\
donald trump    &         191 &     41.4 &                 3.2 &               4.2 &  \cellcolor[rgb]{0.978,0.931,0.956} -0.08 &  \cellcolor[rgb]{0.962,0.968,0.954} +0.02 \\
bernie          &         170 &     64.1 &                 4.4 &               2.3 &  \cellcolor[rgb]{0.972,0.956,0.964} -0.03 &  \cellcolor[rgb]{0.976,0.942,0.959} -0.06 \\
people          &         161 &     54.0 &                 3.6 &               2.8 &  \cellcolor[rgb]{0.965,0.968,0.960} +0.01 &  \cellcolor[rgb]{0.962,0.968,0.954} +0.02 \\
obama           &         155 &     63.2 &                 4.0 &               2.1 &  \cellcolor[rgb]{0.972,0.956,0.964} -0.03 &  \cellcolor[rgb]{0.957,0.967,0.942} +0.04 \\
campaign        &         134 &     67.2 &                 3.7 &               1.6 &  \cellcolor[rgb]{0.959,0.968,0.948} +0.03 &  \cellcolor[rgb]{0.973,0.953,0.963} -0.04 \\
bernie sanders  &         126 &     58.7 &                 3.0 &               1.9 &  \cellcolor[rgb]{0.974,0.949,0.962} -0.05 &  \cellcolor[rgb]{0.975,0.946,0.961} -0.05 \\
til             &         125 &     17.6 &                 0.9 &               3.8 &  \cellcolor[rgb]{0.988,0.893,0.942} -0.16 &  \cellcolor[rgb]{0.915,0.962,0.846} +0.16 \\
president       &         124 &     50.0 &                 2.5 &               2.3 &  \cellcolor[rgb]{0.970,0.963,0.967} -0.01 &  \cellcolor[rgb]{0.970,0.963,0.967} -0.01 \\
news            &         123 &     43.9 &                 2.2 &               2.6 &  \cellcolor[rgb]{0.962,0.968,0.954} +0.02 &  \cellcolor[rgb]{0.952,0.967,0.930} +0.05 \\
trumps          &         120 &     39.2 &                 1.9 &               2.7 &  \cellcolor[rgb]{0.977,0.935,0.957} -0.07 &  \cellcolor[rgb]{0.954,0.967,0.936} +0.04 \\
\ignore{
police          &         115 &     52.2 &                 2.4 &               2.1 &  \cellcolor[rgb]{0.952,0.967,0.930} +0.05 &  \cellcolor[rgb]{0.972,0.956,0.964} -0.02 \\
white           &         106 &     50.0 &                 2.2 &               2.0 &  \cellcolor[rgb]{0.962,0.968,0.954} +0.02 &  \cellcolor[rgb]{0.972,0.956,0.964} -0.03 \\
man             &         103 &     30.1 &                 1.3 &               2.7 &  \cellcolor[rgb]{0.969,0.967,0.968} -0.01 &  \cellcolor[rgb]{0.949,0.966,0.924} +0.06 \\
wikileaks       &          95 &     88.4 &                 3.4 &               0.4 &  \cellcolor[rgb]{0.941,0.965,0.906} +0.09 &  \cellcolor[rgb]{0.977,0.935,0.957} -0.08 \\
vote            &          93 &     49.5 &                 1.9 &               1.8 &  \cellcolor[rgb]{0.967,0.968,0.966} +0.01 &  \cellcolor[rgb]{0.967,0.968,0.966} +0.00 \\
state           &          92 &     62.0 &                 2.3 &               1.3 &  \cellcolor[rgb]{0.967,0.968,0.966} +0.00 &  \cellcolor[rgb]{0.972,0.956,0.964} -0.03 \\
russia          &          89 &     53.9 &                 2.0 &               1.5 &  \cellcolor[rgb]{0.946,0.966,0.918} +0.06 &  \cellcolor[rgb]{0.984,0.910,0.948} -0.13 \\
dont            &          88 &     59.1 &                 2.1 &               1.3 &  \cellcolor[rgb]{0.969,0.967,0.968} -0.00 &  \cellcolor[rgb]{0.971,0.960,0.966} -0.02 \\
could           &          87 &     44.8 &                 1.6 &               1.8 &  \cellcolor[rgb]{0.976,0.939,0.958} -0.07 &  \cellcolor[rgb]{0.959,0.968,0.948} +0.02 \\
one             &          86 &     53.5 &                 1.9 &               1.5 &  \cellcolor[rgb]{0.972,0.956,0.964} -0.03 &  \cellcolor[rgb]{0.965,0.968,0.960} +0.01 \\
would           &          86 &     46.5 &                 1.6 &               1.7 &  \cellcolor[rgb]{0.967,0.968,0.966} +0.01 &  \cellcolor[rgb]{0.965,0.968,0.960} +0.01 \\
}
\bottomrule
\end{tabular}

==> figs/unagg_correlations_table_0.2threshold.tex <==

\newcommand{}[1]{}

\small%\footnotesize
 
\begin{tabular}{@{\hskip .05cm}cr|lll}
\toprule
%{} & &     \multicolumn{1}{c}{\footnotesize \textit{All}} &                                     \multicolumn{1}{c}{\footnotesize \textit{Trusted}} &   \multicolumn{1}{c}{\footnotesize \textit{Deceptive}} \\

{} & &     \multicolumn{1}{c}{  \textit{All}} &                                     \multicolumn{1}{c}{ \textit{T Posts}} &   \multicolumn{1}{c}{  \textit{D Posts}} \\
%
\midrule \multirow{7}{*}{\rot{\bf \large \textit{Author's} }} & \multicolumn{1}{l|}{ \textit{  Bias  } } \\
%%\midrule \multirow{10}{*}{\rot{\bf \it \footnotesize Author's Characteristics}} & \multicolumn{1}{l|}{ \textit{ \footnotesize Bias  } } \\

{} & \% Center Right Bias Links & \cellcolor[rgb]{0.860,0.942,0.747} \bf +0.25$\ddag$ & \cellcolor[rgb]{0.969,0.967,0.968} -0.00 & \cellcolor[rgb]{0.831,0.930,0.702} \bf +0.27$\ddag$ \\
%\cline{2-5} {} 
& \multicolumn{1}{l|}{ \textit{   Categorical  } } \\

{

{} & \% Unlabeled Links (Volkova) & \cellcolor[rgb]{0.983,0.914,0.950} -0.12$\ddag$ & \cellcolor[rgb]{0.977,0.935,0.957} -0.07$\ddag$ & \cellcolor[rgb]{0.988,0.866,0.931} \bf -0.21$\ddag$ \\
{} & \% Trusted Links (Volkova) & \cellcolor[rgb]{0.988,0.866,0.931} \bf -0.21$\ddag$ & \cellcolor[rgb]{0.949,0.966,0.924} +0.06$\ddag$ & \cellcolor[rgb]{0.949,0.966,0.924} +0.06$\ddag$ \\

}

{} & \textcolor{white}{....} \% Propaganda Links (Volkova) & \cellcolor[rgb]{0.760,0.899,0.588} \bf +0.35$\ddag$ & \cellcolor[rgb]{0.941,0.965,0.906} +0.08$\ddag$ & \cellcolor[rgb]{0.895,0.958,0.804}  +0.20$\ddag$ \\
{} & \% Questionable Links (MBFC) & \cellcolor[rgb]{0.753,0.896,0.577} \bf +0.37$\ddag$ & \cellcolor[rgb]{0.936,0.965,0.894} +0.10$\ddag$ & \cellcolor[rgb]{0.895,0.958,0.804}  +0.20$\ddag$ \\
%\cline{2-5} {} 
& \multicolumn{1}{l|}{ \textit{   Factualness  } } \\
{} & \% Very Low Factual Links & \cellcolor[rgb]{0.782,0.908,0.622} \bf +0.33$\ddag$ & \cellcolor[rgb]{0.946,0.966,0.918} +0.07$\ddag$ & \cellcolor[rgb]{0.824,0.927,0.691} \bf +0.29$\ddag$ \\

{

{} & \% High Factual Links & \cellcolor[rgb]{0.988,0.866,0.931} \bf -0.21$\ddag$ & \cellcolor[rgb]{0.952,0.967,0.930} +0.05$\ddag$ & \cellcolor[rgb]{0.974,0.949,0.962} -0.04$\dag$ \\

}

\midrule \multirow{14}{*}{\rot{\bf \large \textit{Community's}}} & \multicolumn{1}{l|}{ \textit{   Bias  } } \\
%\midrule \multirow{36}{*}{\rot{\bf \it \footnotesize Community's Characteristics}} & \multicolumn{1}{l|}{ \textit{ \footnotesize Bias  } } \\

%{} & \# Center Bias Links & \cellcolor[rgb]{0.910,0.962,0.834} +0.17$\ddag$ & \cellcolor[rgb]{0.912,0.962,0.840} +0.17$\ddag$ & \cellcolor[rgb]{0.902,0.961,0.816}  +0.20$\ddag$ \\
{} & \# Right Bias Links & \cellcolor[rgb]{0.860,0.942,0.747} \bf +0.25$\ddag$ & \cellcolor[rgb]{0.907,0.961,0.828} +0.18$\ddag$ & \cellcolor[rgb]{0.941,0.965,0.906} +0.08$\ddag$ \\

{

{} & \# Extreme Right Bias Links & \cellcolor[rgb]{0.874,0.948,0.770} \bf +0.23$\ddag$ & \cellcolor[rgb]{0.918,0.963,0.852} +0.15$\ddag$ & \cellcolor[rgb]{0.954,0.967,0.936} +0.04$\dag$ \\

{} & \# Unlabeled Bias Links & \cellcolor[rgb]{0.895,0.958,0.804} \bf +0.21$\ddag$ & \cellcolor[rgb]{0.944,0.966,0.912} +0.08$\ddag$ & \cellcolor[rgb]{0.941,0.965,0.906} +0.08$\ddag$ \\

}

%\cline{2-5} {} 
& \multicolumn{1}{l|}{ \textit{   Categorical  } } \\

{

{} & \# Retired Links (MBFC) & \cellcolor[rgb]{0.881,0.952,0.782} \bf +0.23$\ddag$ & \cellcolor[rgb]{0.910,0.962,0.834} +0.17$\ddag$ & \cellcolor[rgb]{0.954,0.967,0.936} +0.05$\ddag$ \\

}

{} & \# Clickbait Links (Volkova) & \cellcolor[rgb]{0.860,0.942,0.747} \bf +0.25$\ddag$ & \cellcolor[rgb]{0.912,0.962,0.840} +0.17$\ddag$ & \cellcolor[rgb]{0.949,0.966,0.924} +0.06$\ddag$ \\

{

{} & \# Hoax Links (Volkova) & \cellcolor[rgb]{0.888,0.955,0.793} \bf +0.22$\ddag$ & \cellcolor[rgb]{0.931,0.964,0.882} +0.12$\ddag$ & \cellcolor[rgb]{0.944,0.966,0.912} +0.08$\ddag$ \\
{} & \# Propaganda Links (Volkova) & \cellcolor[rgb]{0.874,0.948,0.770} \bf +0.23$\ddag$ & \cellcolor[rgb]{0.925,0.964,0.870} +0.13$\ddag$ & \cellcolor[rgb]{0.931,0.964,0.882} +0.11$\ddag$ \\
{} & \# Conspiracy Links (MBFC) & \cellcolor[rgb]{0.874,0.948,0.770} \bf +0.23$\ddag$ & \cellcolor[rgb]{0.920,0.963,0.858} +0.14$\ddag$ & \cellcolor[rgb]{0.949,0.966,0.924} +0.05$\ddag$ \\

}

{} & \# Questionable Links (MBFC) & \cellcolor[rgb]{0.845,0.936,0.725} \bf +0.26$\ddag$ & \cellcolor[rgb]{0.910,0.962,0.834} +0.18$\ddag$ & \cellcolor[rgb]{0.944,0.966,0.912} +0.08$\ddag$ \\

{

{} & \% Questionable Links (MBFC) & \cellcolor[rgb]{0.881,0.952,0.782} \bf +0.23$\ddag$ & \cellcolor[rgb]{0.902,0.961,0.816} +0.20$\ddag$ & \cellcolor[rgb]{0.967,0.968,0.966} +0.00 \\

{} & \# Unlabeled Links (Volkova) & \cellcolor[rgb]{0.888,0.955,0.793} \bf +0.21$\ddag$ & \cellcolor[rgb]{0.936,0.965,0.894} +0.10$\ddag$ & \cellcolor[rgb]{0.941,0.965,0.906} +0.08$\ddag$ \\
{} & \# Unlabeled Links (MBFC) & \cellcolor[rgb]{0.895,0.958,0.804} \bf +0.21$\ddag$ & \cellcolor[rgb]{0.944,0.966,0.912} +0.08$\ddag$ & \cellcolor[rgb]{0.941,0.965,0.906} +0.08$\ddag$ \\

}

%\cline{2-5} {} 
& \multicolumn{1}{l|}{ \textit{  Factualness  } } \\
{} & \# Very Low Factual Links & \cellcolor[rgb]{0.803,0.918,0.656} \bf +0.31$\ddag$ & \cellcolor[rgb]{0.918,0.963,0.852} +0.15$\ddag$ & \cellcolor[rgb]{0.910,0.962,0.834} +0.17$\ddag$ \\

{

{} & \% Very Low Factual Links & \cellcolor[rgb]{0.895,0.958,0.804} \bf +0.21$\ddag$ & \cellcolor[rgb]{0.920,0.963,0.858} +0.14$\ddag$ & \cellcolor[rgb]{0.928,0.964,0.876} +0.12$\ddag$ \\

}

{} & \# Low Factual Links & \cellcolor[rgb]{0.860,0.942,0.747} \bf +0.25$\ddag$ & \cellcolor[rgb]{0.915,0.962,0.846} +0.16$\ddag$ & \cellcolor[rgb]{0.944,0.966,0.912} +0.07$\ddag$ \\

{

{} & \# Mixed Factual Links & \cellcolor[rgb]{0.867,0.945,0.759} \bf +0.24$\ddag$ & \cellcolor[rgb]{0.907,0.961,0.828} +0.18$\ddag$ & \cellcolor[rgb]{0.939,0.965,0.900} +0.09$\ddag$ \\

{} & \% Mixed Factual Links & \cellcolor[rgb]{0.907,0.961,0.828} +0.18$\ddag$ & \cellcolor[rgb]{0.895,0.958,0.804} \bf +0.21$\ddag$ & \cellcolor[rgb]{0.971,0.960,0.966} -0.02 \\


{} & \# Very High Factual Links & \cellcolor[rgb]{0.918,0.963,0.852} +0.15$\ddag$ & \cellcolor[rgb]{0.923,0.963,0.864} +0.14$\ddag$ & \cellcolor[rgb]{0.867,0.945,0.759} \bf +0.24$\ddag$ \\

{} & \# Unlabeled Factualness Links & \cellcolor[rgb]{0.895,0.958,0.804} \bf +0.21$\ddag$ & \cellcolor[rgb]{0.944,0.966,0.912} +0.08$\ddag$ & \cellcolor[rgb]{0.941,0.965,0.906} +0.08$\ddag$ \\

}

%\cline{2-5}  {} 

{


& \multicolumn{1}{l|}{ \textit{  General  } } \\ 
{} & \# Posts & \cellcolor[rgb]{0.881,0.952,0.782} \bf +0.22$\ddag$ & \cellcolor[rgb]{0.928,0.964,0.876} +0.12$\ddag$ & \cellcolor[rgb]{0.939,0.965,0.900} +0.09$\ddag$ \\
%{} & \# Selfposts & \cellcolor[rgb]{0.895,0.958,0.804} +0.20$\ddag$ & \cellcolor[rgb]{0.944,0.966,0.912} +0.07$\ddag$ & \cellcolor[rgb]{0.949,0.966,0.924} +0.06$\ddag$ \\
{} & \# Linkposts & \cellcolor[rgb]{0.881,0.952,0.782} \bf +0.22$\ddag$ & \cellcolor[rgb]{0.931,0.964,0.882} +0.12$\ddag$ & \cellcolor[rgb]{0.933,0.964,0.888} +0.10$\ddag$ \\
{} & \# Deleted Posts & \cellcolor[rgb]{0.888,0.955,0.793} \bf +0.22$\ddag$ & \cellcolor[rgb]{0.925,0.964,0.870} +0.13$\ddag$ & \cellcolor[rgb]{0.944,0.966,0.912} +0.07$\ddag$ \\
{} & \# Links & \cellcolor[rgb]{0.888,0.955,0.793} \bf +0.22$\ddag$ & \cellcolor[rgb]{0.928,0.964,0.876} +0.12$\ddag$ & \cellcolor[rgb]{0.939,0.965,0.900} +0.09$\ddag$ \\
{} & \# Twitter Links & \cellcolor[rgb]{0.867,0.945,0.759} \bf +0.24$\ddag$ & \cellcolor[rgb]{0.931,0.964,0.882} +0.11$\ddag$ & \cellcolor[rgb]{0.933,0.964,0.888} +0.10$\ddag$ \\
{} & \# Potential News Links & \cellcolor[rgb]{0.888,0.955,0.793} \bf +0.21$\ddag$ & \cellcolor[rgb]{0.928,0.964,0.876} +0.12$\ddag$ & \cellcolor[rgb]{0.918,0.963,0.852} +0.15$\ddag$ \\
{} & \# Non-News Social Links & \cellcolor[rgb]{0.888,0.955,0.793} \bf +0.22$\ddag$ & \cellcolor[rgb]{0.936,0.965,0.894} +0.09$\ddag$ & \cellcolor[rgb]{0.944,0.966,0.912} +0.07$\ddag$ \\
%{} & \% Non-News Reference Links & \cellcolor[rgb]{0.988,0.896,0.943} -0.16$\ddag$ & \cellcolor[rgb]{0.992,0.878,0.937}  -0.20$\ddag$ & \cellcolor[rgb]{0.988,0.896,0.943} -0.16$\ddag$ \\
%{} & \# Non-News External Host Links & \cellcolor[rgb]{0.895,0.958,0.804} +0.20$\ddag$ & \cellcolor[rgb]{0.941,0.965,0.906} +0.08$\ddag$ & \cellcolor[rgb]{0.957,0.967,0.942} +0.04$\dag$ \\

}

%\cline{2-5} {} 
& \multicolumn{1}{l|}{ \textit{  Inequality  } } \\
{} & Gini Coefficient (\# Links) & \cellcolor[rgb]{0.796,0.915,0.645} \bf +0.32$\ddag$ & \cellcolor[rgb]{0.910,0.962,0.834} +0.18$\ddag$ & \cellcolor[rgb]{0.925,0.964,0.870} +0.13$\ddag$ \\
\midrule 
%\multicolumn{1}{l}{ \rot{ \it Post  } }
& Post Score & \cellcolor[rgb]{0.928,0.964,0.876} +0.12$\ddag$ & \cellcolor[rgb]{0.978,0.931,0.956} -0.08$\ddag$ & \cellcolor[rgb]{0.845,0.936,0.725} {\bf +0.27$\ddag$} \\ \midrule
\end{tabular}
